The accuracy of the UV continuum as an indicator of the star formation rate in galaxies

The rest-frame intrinsic UV luminosity is often used as an indicator of the instantaneous star formation rate (SFR) in a galaxy. While it is in general a robust indicator of the ongoing star formation activity, the precise value of the calibration relating the UV luminosity to the SFR ($B_{\nu}$), is sensitive to various physical properties, such as the recent star formation and metal enrichment histories, along with the choice of stellar initial mass function. The distribution of these properties for the star-forming galaxy population then suggests that the adoption of a single calibration is not appropriate unless properly qualified with the uncertainties on the calibration. We investigate, with the aid of the {\sc galform} semi-analytic model of galaxy formation, the distribution of UV-SFR calibrations obtained using realistic star formation and metal enrichment histories. At $z=0$, we find that when the initial mass function is fixed (to the Kennicutt IMF), the median calibration is $B_{\rm fuv}=0.9$ where ${\rm SFR}/[{\rm M_{\odot}\,yr^{-1}}]=B_{\nu}\times 10^{-28}\times L_{\nu}/[{\rm ergs\,s^{-1}\,Hz^{-1}}]$. However, the width of the distribution $B_{\rm fuv}$ suggests that for a single object there is around a 20% {\em intrinsic} uncertainty (at $z=0$, rising to $\simeq 30%$ at $z=6$) on the star formation rate inferred from the FUV luminosity without additional constraints on the star formation history or metallicity. We also find that the median value of the calibration $B_{\rm fuv}$ is correlated with the star formation rate and redshift (at $z>3$) raising implications for the correct determination of the star formation rate from the UV.

==> PaxHeader/paper.tex <==
18 uid=1258190603
20 ctime=1347790409
20 atime=1347790409
24 SCHILY.dev=234881028
23 SCHILY.ino=10832946
18 SCHILY.nlink=1

